Deep Learning Based Cryptographic Primitive Classification

Cryptovirological augmentations present an immediate, incomparable threat. Over the last decade, the substantial proliferation of crypto-ransomware has had widespread consequences for consumers and organisations alike. Established preventive measures perform well, however, the problem has not ceased. Reverse engineering potentially malicious software is a cumbersome task due to platform eccentricities and obfuscated transmutation mechanisms, hence requiring smarter, more efficient detection strategies. The following manuscript presents a novel approach for the classification of cryptographic primitives in compiled binary executables using deep learning. The model blueprint, a DCNN, is fittingly configured to learn from variable-length control flow diagnostics output from a dynamic trace. To rival the size and variability of contemporary data compendiums, hence feeding the model cognition, a methodology for the procedural generation of synthetic cryptographic binaries is defined, utilising core primitives from OpenSSL with multivariate obfuscation, to draw a vastly scalable distribution. The library, CryptoKnight, rendered an algorithmic pool of AES, RC4, Blowfish, MD5 and RSA to synthesis combinable variants which are automatically fed in its core model. Converging at 91% accuracy, CryptoKnight is successfully able to classify the sample algorithms with minimal loss.

==> confusion-external.tex <==
\begin{center}
	\begin{tabular}{c|ccccc|}  
		%\multicolumn{6}{r}{Predicted} \\
		%\cmidrule(r){1-2}
				& AES & RC4 & BLF & MD5 & RSA \\
		\hhline{------}
		AES		& 2\cellcolor[gray]{.8}			& 0	& 1	& 2	& 0		\\
		RC4		& 1	 & 3\cellcolor[gray]{.8}		& 0	& 1	& 0		\\
		BLF 	& 1	 & 4 & 0\cellcolor[gray]{.8}		& 0	& 0		\\
		MD5		& 2	 & 1 & 0 & 2\cellcolor[gray]{.8}		& 0		\\
		RSA		& 2  & 0 & 1 & 2	& 0\cellcolor[gray]{.8}	 		\\
		\hhline{~-----}
	\end{tabular}
	\captionof{table}{Open Source Verification}
	\label{tbl:github}
	\medskip
	\small
	$x = predicted, y = actual$
\end{center}


==> confusion.tex <==
\begin{table}[h]\centering
	\begin{tabular}{c|cccccc|}  
		%\multicolumn{6}{r}{Predicted} \\
		%\cmidrule(r){1-2}
				& AES & RC4 & BLF & MD5 & RSA & R/A \\
		\hhline{-------}
		AES		& 37\cellcolor[gray]{.8}		& 0	& 0	& 0	& 13 & 0	\\
		RC4		& 0	 & 50\cellcolor[gray]{.8}		& 0	& 0	& 0	 & 0	\\
		BLF 	& 0	 & 8 & 42\cellcolor[gray]{.8}		& 0	& 0	 & 0	\\
		MD5		& 0	 & 2 & 7 & 41\cellcolor[gray]{.8}		& 0	 & 0	\\
		RSA		& 19 & 0 & 0 & 0	& 30\cellcolor[gray]{.8}	 & 1	\\
		R/A		& 0	 & 0 & 0 & 0	& 0	& 50\cellcolor[gray]{.8}		\\
		\hhline{~------}
	\end{tabular}
	\caption{Confusion Matrix}
	\label{tbl:confusion}
	\medskip
	\small
	$x = predicted, y = actual$
\end{table}

